Semialgebraic groups and generalized affine buildings

We develop the theory of algebraic groups over real closed fields and apply the results to construct a geometric object $\mathcal{B}$ and to prove that $\mathcal{B}$ is an affine $\Lambda$-building. We use a model theoretic transfer principle to prove generalizations of statements about semisimple Lie groups. In this direction we give proofs for the Iwasawa-decomposition $KAU$, the Cartan-decomposition $KAK$ and the Bruhat-decomposition $BWB$. For unipotent subgroups we prove the Baker-Campbell-Hausdorff formula and use it to analyse root groups. We give a proof of the Jacobson-Morozov Lemma about subgroups whose Lie algebra is isomorphic to $\mathfrak{sl}_2$ and we describe other rank 1 subgroups which are the semisimple parts of Levi-subgroups. We prove a semialgebraic version of Kostant's convexity. Over the reals, semisimple Lie groups are closely related to the symmetry groups of symmetric spaces of non-compact type. These symmetric spaces can be described semialgebraically, which allows us to consider their semialgebraic extension over any real closed field. Starting from these non-standard symmetric spaces we use a valuation (with image some non-discrete ordered abelian group $\Lambda$) on the fields to define a $\Lambda$-pseudometric. Identifying points of distance zero results in a $\Lambda$-metric space $\mathcal{B}$. Assuming that the root system of the associated Lie group is reduced, we prove that $\mathcal{B}$ is an affine $\Lambda$-building. The proof relies on a thorough analysis of stabilizers.

==> figures/tikzpaper/buildings_diagram_v0.1 <==
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=none] (0) at (-13, 7) {};
		\node [style=none] (1) at (-14, 6) {};
		\node [style=none] (2) at (-14, 1) {};
		\node [style=none] (3) at (-13, 0) {};
		\node [style=none] (4) at (-8, 0) {};
		\node [style=none] (5) at (-7, 1) {};
		\node [style=none] (6) at (-7, 6) {};
		\node [style=none] (7) at (-8, 7) {};
		\node [style=none] (9) at (-10.5, 7.75) {simplicial buildings};
		\node [style=none] (11) at (-11, 4) {spherical \newline buildings};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (0.center) to (7.center);
		\draw [bend left=45, looseness=1.75] (7.center) to (6.center);
		\draw (6.center) to (5.center);
		\draw [bend left=45, looseness=1.75] (5.center) to (4.center);
		\draw (4.center) to (3.center);
		\draw [bend left=45, looseness=1.75] (3.center) to (2.center);
		\draw (2.center) to (1.center);
		\draw [bend left=45, looseness=1.75] (1.center) to (0.center);
	\end{pgfonlayer}
\end{tikzpicture}

